AutoMLBench: A Comprehensive Experimental Evaluation of Automated Machine Learning Frameworks

With the booming demand for machine learning applications, it has been recognized that the number of knowledgeable data scientists can not scale with the growing data volumes and application needs in our digital world. In response to this demand, several automated machine learning (AutoML) frameworks have been developed to fill the gap of human expertise by automating the process of building machine learning pipelines. Each framework comes with different heuristics-based design decisions. In this study, we present a comprehensive evaluation and comparison of the performance characteristics of six popular AutoML frameworks, namely, AutoWeka, AutoSKlearn, TPOT, Recipe, ATM, and SmartML, across 100 data sets from established AutoML benchmark suites. Our experimental evaluation considers different aspects for its comparison, including the performance impact of several design decisions, including time budget, size of search space, meta-learning, and ensemble construction. The results of our study reveal various interesting insights that can significantly guide and impact the design of AutoML frameworks.

==> tables/commented-figures.tex <==

\iffalse
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Figures/F1Differencebetweenfcand3cfor30minutesAutoSKLearn.pdf}
  \caption{The impact of search space size - AutoSKLearn}
  \label{fig:ss_autosklearn}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Figures/F1Differencebetweenfcand3cfor30minutesTPOT.pdf}
  \caption{The impact of search space size - TPOT}
  \label{fig:ss_tpot}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Figures/F1Differencebetweenfcand3cfor30minutesATM.pdf}
  \caption{The impact of search space size - ATM}
  \label{fig:ss_atml}
\end{figure}
\fi


==> tables/commented-tables.tex <==


\iffalse
Tables \ref{tab:wilcoxon_timebudget_autosklearn_e}, \ref{tab:wilcoxon_timebudget_autosklearn_m}, \ref{tab:wilcoxon_timebudget_autosklearn_v}, \ref{tab:wilcoxon_timebudget_autoweka}, \ref{tab:wilcoxon_timebudget_recipe}, and \ref{tab:wilcoxon_timebudget_smartml} summarizes the results for the rest of \texttt{autoML} frameworks. In general, increasing the time budget can produce a successful run, boost the performance accuracy, or decline it. As we have noticed from the results of the special runs that are repeated 3 times for the outlier datasets, the datasets \texttt{tumors\_C, CovPokElec, dbworld-bodies} and others have repeated behavior with extreme accuracy of their pipelines. Most of these repeated datasets have a number of instances less than 50\% of the datasets and a number of features more than 50\% of the datasets. So, we have tried to build a linear regression model based on the datasets' meta-features to predict the expected accuracy and variance, given the time budget. The predicted accuracy for the time budget options can be considered as a heuristic to balance the trade-off between accuracy gain and resource consumption. The expected variance of these datasets within the selected time budget helps to decide if extra repeated runs are required or not. The linear regression model is interpretable, so it may give insights about the important meta-features.


For each time budget in our experiment, i.e 10, 30, 60 and 240 minutes, a linear regression model is defined as follows:
$$ Acc(\alpha) = \sum_{i=1}^{n} \alpha_{i} \theta_{i}$$
Where $\alpha_{i}$ is the $i^{th}$ meta-feature, $\alpha$ is the meta-feature vector, $ \theta_{i}$ is the $i^{th}$ learned model parameter and $Acc(\alpha)$ is the predicted accuracy for the data set that has $\alpha$ as its meta-feature vector.

The model is trained over 80\% of the successful runs within the target time budget and the training error is computed for the training samples ($E_i$). The standard deviation of these training errors can be calculated as follows:
$$\sigma = \sqrt{\frac{ \sum_{i=1}^{n} E_i}{n-1}}$$
The prediction intervals that correspond to 95\% of confidence level is computed as follows:
$$I = 1.96 * \sigma$$
Where 1.96 is the approximate value of the 97.5 percentile point of the normal distribution. 95\% of the area under a normal curve lies within roughly 1.96 standard deviations of the mean, and due to the central limit theorem, this number is therefore used in the construction of approximate 95\% confidence intervals. Therefore the expected accuracy interval can be considered as $Acc(\alpha) \pm I$. Figure \ref{fig:tb_model} shows the results of the expected accuracy, expected intervals, true accuracy within 10 minutes time budget.
\fi



\iffalse
\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - AutoSkLearn-e}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    AutoSKLearn-e&    30&    10& 0.007 &    \textbf{0.000}\\
    \hline
    AutoSKLearn-e&    60&    10& 0.011 &    \textbf{0.000}\\
    AutoSKLearn-e&    60&    30& 0.004 &    0.675\\
    \hline
    AutoSKLearn-e&    240&    10& 0.013 &    \textbf{0.000}\\
    AutoSKLearn-e&    240&    30& 0.006 & \textbf{0.038}\\
    AutoSKLearn-e&    240&    60& 0.002 & 0.265\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_autosklearn_e}
\end{table}

\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - AutoSkLearn-m}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    AutoSKLearn-m&    30&    10& 0.004  &    0.211\\
    \hline
    AutoSKLearn-m&    60&    10& 0.004  &    0.198\\
    AutoSKLearn-m&    60&    30& 0.00  &    0.956\\
    \hline
    AutoSKLearn-m&    240&    10& 0.008  &    0.099\\
    AutoSKLearn-m&    240&    30& 0.004  & 0.614\\
    AutoSKLearn-m&    240&    60& 0.004  & 0.398\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_autosklearn_m}
\end{table}


\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - AutoSkLearn-v}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    AutoSKLearn-v&    30&    10& 0.005 &    0.226\\
    \hline
    AutoSKLearn-v&    60&    10& 0.007 &    \textbf{0.004}\\
    AutoSKLearn-v&    60&    30& 0.002 &    0.141\\
    \hline
    AutoSKLearn-v&    240&    10& 0.007 &    \textbf{0.000}\\
    AutoSKLearn-v&    240&    30& 0.002 & \textbf{0.027}\\
    AutoSKLearn-v&    240&    60& 0.000 & 0.110\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_autosklearn_v}
\end{table}


\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - AutoWeka}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    AutoWeka&    30&    10& 0.031 &    \textbf{0.005}\\
    \hline
    AutoWeka&    60&    10& 0.038 &    \textbf{0.037}\\
    AutoWeka&    60&    30&     0.008 &0.658\\
    \hline
    AutoWeka&    240&    10& 0.083 &    \textbf{0.000}\\
    AutoWeka&    240&    30& 0.051 & \textbf{0.022}\\
    AutoWeka&    240&    60& 0.044 & \textbf{0.004}\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_autoweka}
\end{table}


\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - Recipe}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    Recipe&    30&    10& -0.031 &    0.272\\
    \hline
    Recipe&    60&    10& 0.014 &0.067\\
    Recipe&    60&    30& 0.007 &    0.829\\
    \hline
    Recipe&    240&    10& 0.026 &    \textbf{0.010}\\
    Recipe&    240&    30& 0.005 & 0.650\\
    Recipe&    240&    60& -0.001 & 0.939\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_recipe}
\end{table}


\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - SmartML}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    Recipe&    30&    10& 0.007 &    0.636\\
    \hline
    Recipe&    60&    10& 0.009 &0.832\\
    Recipe&    60&    30& 0.009 &    0.597\\
    \hline
    Recipe&    240&    10& 0.026 &    0.121\\
    Recipe&    240&    30& 0.025 & \textbf{0.050}\\
    Recipe&    240&    60& 0.015 & 0.071\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_smartml}
\end{table}


\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - TPOT}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    Recipe&    30&    10& 0.009 &    0.165\\
    \hline
    Recipe&    60&    10& 0.008 &0.399\\
    Recipe&    60&    30& 0.001 &    0.400\\
    \hline
    Recipe&    240&    10& 0.013 &    \textbf{0.013}\\
    Recipe&    240&    30& 0.006 & \textbf{0.027}\\
    Recipe&    240&    60& 0.004 & \textbf{0.010}\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_tpot}
\end{table}


\begin{table}[t]
\begin{center}
\caption{The Results of Wilcoxon Test for Assessing the Significance on Performance Difference by increasing the time budget - ATM}
\begin{tabular}{ |c|c|c|c|c| }
  \hline

    Framework &TB1& Time Budget2 &Avg. Acc. Diff& P value \\
     \hline
    Recipe&    30&    10& 0.007 &    0.341\\
    \hline
    Recipe&    60&    10& 0.009 &0.488\\
    Recipe&    60&    30& 0.009 &    0.538\\
    \hline
    Recipe&    240&    10& 0.026 &    0.594\\
    Recipe&    240&    30& 0.025 & 0.964\\
    Recipe&    240&    60& 0.015 & 0.496\\
 \hline
\end{tabular}
\end{center}
\label{tab:wilcoxon_timebudget_atm}
\end{table}
\fi



\iffalse
% \begin{table*}[t]
% \begin{center}
% \caption{Result Summary}
% \begin{tabular}{ |c|c|c|c|c|c|cc| }
%   \hline


%     Time Budget &    Framework & N &    Mean &    SD &    SE &    [95\% Conf. &    Interval]         \\
%      \hline
%     \multirow{9}{*}{10} & ATM &  75 &  0.888 &  0.123 &  0.014 &      0.860 &     0.916 \\
%     & Autoweka &  86 &  0.848 &  0.161 &  0.017 &      0.814 &     0.882 \\
%     & Recipe &  33 &  0.840 &  0.176 &  0.031 &      0.780 &     0.900 \\
%     & AutoSKLearn-e &  99 &  0.873 &  0.139 &  0.014 &      0.846 &     0.901 \\
%     & AutoSKLearn-m &  99 &  0.870 &  0.144 &  0.015 &      0.841 &     0.898 \\
%     & AutoSKLearn-v &  99 &  0.868 &  0.145 &  0.015 &      0.839 &     0.896 \\
%     &AutoSKLearn &  99 &  0.873 &  0.143 &  0.014 &      0.845 &     0.901 \\
%     & SmartML &  89 &  0.799 &  0.212 &  0.022 &      0.755 &     0.843 \\
%     & TPOT &  43 &  0.894 &  0.117 &  0.018 &      0.859 &     0.929 \\
%     \hline
%     \multirow{9}{*}{30} & ATM &  74 &  0.903 &  0.116 &  0.013 &      0.877 &     0.930 \\
%     & Autoweka &  90 &  0.845 &  0.161 &  0.017 &      0.812 &     0.878 \\
%     & Recipe &  69 &  0.855 &  0.144 &  0.017 &      0.821 &     0.889 \\
%     & AutoSKLearn-e &  99 &  0.880 &  0.136 &  0.014 &      0.854 &     0.907 \\
%     & AutoSKLearn-m &  99 &  0.873 &  0.143 &  0.014 &      0.845 &     0.901 \\
%     & AutoSKLearn-v &  99 &  0.873 &  0.142 &  0.014 &      0.845 &     0.901 \\
%     &AutoSKLearn &  98 &  0.879 &  0.138 &  0.014 &      0.851 &     0.906 \\
%     & SmartML &  90 &  0.808 &  0.199 &  0.021 &      0.767 &     0.849 \\
%     & TPOT &  59 &  0.885 &  0.136 &  0.018 &      0.850 &     0.920 \\
%     \hline
%     \multirow{9}{*}{60} & ATM &  79 &  0.890 &  0.126 &  0.014 &      0.862 &     0.918 \\
%     & Autoweka &  91 &  0.844 &  0.157 &  0.017 &      0.811 &     0.876 \\
%     & Recipe &  76 &  0.864 &  0.139 &  0.016 &      0.833 &     0.895 \\
%     & AutoSKLearn-e &  99 &  0.884 &  0.132 &  0.013 &      0.858 &     0.910 \\
%     & AutoSKLearn-m &  99 &  0.873 &  0.141 &  0.014 &      0.846 &     0.901 \\
%     & AutoSKLearn-v &  99 &  0.874 &  0.137 &  0.014 &      0.847 &     0.901 \\
%     &AutoSKLearn &  99 &  0.882 &  0.133 &  0.013 &      0.856 &     0.908 \\
%     & SmartML &  89 &  0.816 &  0.194 &  0.021 &      0.776 &     0.856 \\
%     & TPOT &  70 &  0.890 &  0.131 &  0.016 &      0.859 &     0.920 \\
%     \hline
%     \multirow{9}{*}{240} & ATM &  86 &  0.895 &  0.123 &  0.013 &      0.869 &     0.921 \\
%     & Autoweka &  96 &  0.845 &  0.159 &  0.016 &      0.813 &     0.877 \\
%     & Recipe &  85 &  0.859 &  0.155 &  0.017 &      0.826 &     0.892 \\
%     & AutoSKLearn-e &  97 &  0.888 &  0.128 &  0.013 &      0.862 &     0.913 \\
%     & AutoSKLearn-m &  95 &  0.882 &  0.134 &  0.014 &      0.855 &     0.909 \\
%     & AutoSKLearn-v &  96 &  0.874 &  0.149 &  0.015 &      0.844 &     0.904 \\
%     &AutoSKLearn &  96 &  0.893 &  0.127 &  0.013 &      0.867 &     0.918 \\
%     & SmartML &  89 &  0.826 &  0.169 &  0.018 &      0.791 &     0.862 \\
%     & TPOT &  89 &  0.893 &  0.126 &  0.013 &      0.866 &     0.919 \\
%  \hline
% \end{tabular}
% \end{center}
% \label{tab:summary}
% \end{table*}
\fi

==> tables/time-budget-summary.tex <==
\begin{table}[!ht]
\centering
\caption{Summary of the impact of increasing the time budget. Bold entries highlight highest mean and maximum gain and smallest mean and maximum loss}
% \resizebox{0.9\textwidth}{!}
{\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF}\cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} \textbf{Time Budget}} & & \multicolumn{2}{c}{\textbf{Gain ($g$)}} & \multicolumn{3}{c}{\textbf{\#datasets with}} & \multicolumn{2}{c}{\textbf{Loss ($l$)}} \\
\rowcolor[HTML]{EFEFEF}\cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} in minutes}&  \multirow{-2}{*}{\textbf{Framework}}&  \textbf{Mean} & \textbf{Max} & \textbf{ $g>1\%$} & \textbf{ $g\approx 0 \%$} & \textbf{ $l>1\%$} & \textbf{Mean} & \textbf{Max} \\ \hline
 & \textbf{ATM} &   4.2  &  21.0  &  21  &  33  &  13  &  -4.7  &  -21.0 \\ \cline{2-9}  
 & \textbf{AutoWeka} &   6.1  &  19.6  &  14  &  65  &  7  &  -3.8  &  -11.5 \\ \cline{2-9} 
 & \textbf{Recipe} & \textbf{13.6}  &  25.0  &  2  &  17  &  2  &  -4.1  &  -5.4 \\ \cline{2-9} 
 & \textbf{AutoSKLearn-e} &   3.6  &  13.4  &  24  &  67  &  8  &  -3.4  &  -11.2 \\ \cline{2-9} 
 & \textbf{AutoSKLearn-m}&   3.8  &  12.5  &  19  &  68  &  12  &  -3.0  &  -13.3 \\ \cline{2-9}
 & \textbf{AutoSKLearn-v}&   4.6  &  22.2  &  18  &  69  &  12  &  -2.9  &  -6.2 \\ \cline{2-9} 
 & \textbf{AutoSKLearn}&  3.2  &  13.9  &  17  &  73  &  9  &  -2.3  &  -4.3 \\ \cline{2-9} 
 & \textbf{SmartML}& 8.0  &  33.3  &  13  &  64  &  11  &  -3.6  &  -8.3 \\ \cline{2-9}
 & \textbf{SmartML-e}& 7.9  &  \textbf{85.2}  &  18  &  67  &  11  &  -6.3  &  -16.9 \\ \cline{2-9}
\multirow{-9}{*}{\textbf{$10 \to 30$}} & \textbf{TPOT}&  6.3  &  17.9  &  7  &  28  &  5  &  \textbf{-2.0} & \textbf{-3.7} \\ \hline
 & \textbf{ATM} &  4.5  &  16.7  &  15  &  35  &  19  &  -6.6  &  -25.0 \\ \cline{2-9} 
 & \textbf{AutoWeka} & \textbf{12.4}  &  \textbf{66.6}  &  10  &  66  &  14  &  -8.1  &  -39.9 \\ \cline{2-9} 
 & \textbf{Recipe} & 4.3  &  12.5  &  5  &  59  &  3  &  -12.5  &  -17.8 \\ \cline{2-9} 
 & \textbf{AutoSKLearn-e} &  4.3  &  18.8  &  18  &  66  &  15  &  \textbf{-2.4}  &  \textbf{-6.2} \\ \cline{2-9}
 & \textbf{AutoSKLearn-m}&  4.1  &  12.5  &  14  &  71  &  14  &  -4.1  &  -12.5 \\ \cline{2-9} 
 & \textbf{AutoSKLearn-v}&   3.6  &  12.5  &  23  &  63  &  13  &  -5.1  &  -13.9 \\ \cline{2-9} 
 & \textbf{AutoSKLearn}& 3.6  &  17.1  &  21  &  69  &  9  &  -2.7  &  -6.7 \\ \cline{2-9}  
 & \textbf{SmartML}& 12.2  &  40.0  &  10  &  73  &  6  &  -6.2  &  -18.3 \\ \cline{2-9} 
 & \textbf{SmartML-e}& 6.5  &  18.2  &  21  &  54  &  20  &  -9.0  &  -84.3 \\ \cline{2-9}
\multirow{-9}{*}{\textbf{$30 \to 60$}} & \textbf{TPOT}&   3.7  &  8.9  &  6  &  43  &  7  &  -2.9  &  -7.0 \\ \hline

& \textbf{ATM} &  5.3  &  26.8  &  20  &  41  &  16  &  -4.0  &  -13.9 \\ \cline{2-9} 
& \textbf{AutoWeka} &  4.3  &  10.8  &  17  &  66  &  8  &  -4.4  &  -11.3 \\ \cline{2-9} 
& \textbf{Recipe} &  10.5  &  26.3  &  4  &  70  &  1  &  -37.5  &  -37.5 \\ \cline{2-9} 
& \textbf{AutoSKLearn-e} &  3.8  &  33.4  &  20  &  64  &  15  &  -3.8  &  -12.5 \\ \cline{2-9} 
& \textbf{AutoSKLearn-m}&  4.1  &  12.5  &  19  &  66  &  14  &  \textbf{-2.7}  &  \textbf{-4.9} \\ \cline{2-9}  
& \textbf{AutoSKLearn-v}&  3.1  &  12.5  &  24  &  62  &  13  &  -5.8  &  -16.7 \\ \cline{2-9}  
& \textbf{AutoSKLearn}&  4.3  &  34.5  &  22  &  64  &  13  &  -3.3  &  -10.3 \\ \cline{2-9} 
& \textbf{SmartML}&  \textbf{10.6}  &  \textbf{59.6}  &  19  &  59  &  10  &  -6.6  &  -19.4 \\ \cline{2-9} 
& \textbf{SmartML-e}& 9.1  &  22.3  &  23  &  53  &  19  &  -6.9  &  -18.8 \\ \cline{2-9}
\multirow{-9}{*}{\textbf{$60 \to 240 $}} & \textbf{TPOT}&   2.5  &  5.6  &  19  &  46  &  5  &  -4.1  &  -7.7 \\ \hline

\end{tabular}}
\label{tab:TBSummary}
\end{table}

==> tables/time-budget.tex <==

\begin{table}[!ht]
\centering
\caption{Mean and standard deviation of the accuracy of AutoML frameworks per time budget. Bold entries highlight highest mean and lowest standard deviation}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} \textbf{Time Budget}} & \textbf{Framework} & \textbf{N} & \textbf{Mean} & \textbf{SD} & \cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{Time Budget}} & \textbf{Framework} & \textbf{N} & \textbf{Mean} & SD \\ \hline
 & \textbf{ATM} & 75 & 0.888 & 0.123 &  & \textbf{ATM} & 79 & \textbf{0.891} & \textbf{0.126} \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoWeka} & 86 & 0.848 & 0.161 &  & \textbf{AutoWeka} & 91 & 0.844 & 0.157 \\ \cline{2-5} \cline{7-10} 
 & \textbf{Recipe} & 33 & 0.840 & 0.176 &  & \textbf{Recipe} & 76 & 0.864 & 0.139 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn-e} & 99 & 0.873 & 0.139 &  & \textbf{AutoSKLearn-e} & 99 & 0.884 & 0.132 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn-m} & 99 & 0.870 & 0.144 &  & \textbf{AutoSKLearn-m} & 99 & 0.873 & 0.141 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn-v} & 99 & 0.868 & 0.145 &  & \textbf{AutoSKLearn-v} & 99 & 0.874 & 0.137 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn} & 99 & 0.873 & 0.143 &  & \textbf{AutoSKLearn} & 99 & 0.882 & 0.133 \\ \cline{2-5} \cline{7-10} 
 & \textbf{SmartML} & 89 & 0.799 & 0.212 &  & \textbf{SmartML} & 89 & 0.816 & 0.194 \\ \cline{2-5} \cline{7-10}
 & \textbf{SmartML-e} & 97 & 0.831 & 0.176 &  & \textbf{SmartML-e} & 95 & 0.832 & 0.0172 \\ \cline{2-5} \cline{7-10}
\multirow{-9}{*}{\textbf{10 Min}} & \textbf{TPOT} & 43 & \textbf{0.894} & \textbf{0.117} & \multirow{-9}{*}{\textbf{60 Min}} & \textbf{TPOT} & 70 & 0.890 & 0.131 \\ \hline
 & \textbf{ATM} & 74 & \textbf{0.903} & \textbf{0.116} &  & \textbf{ATM} & 86 & \textbf{0.895} & \textbf{0.123} \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoWeka} & 90 & 0.845 & 0.161 &  & \textbf{AutoWeka} & 96 & 0.845 & 0.159 \\ \cline{2-5} \cline{7-10} 
 & \textbf{Recipe} & 69 & 0.855 & 0.144 &  & \textbf{Recipe} & 85 & 0.859 & 0.155 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn-e} & 99 & 0.880 & 0.136 &  & \textbf{AutoSKLearn-e} & 99 & 0.886 & 0.130 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn-m} & 99 & 0.873 & 0.143 &  & \textbf{AutoSKLearn-m} & 99 & 0.877 & 0.136 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn-v} & 99 & 0.873 & 0.142 &  & \textbf{AutoSKLearn-v} & 99 & 0.875 & 0.141 \\ \cline{2-5} \cline{7-10} 
 & \textbf{AutoSKLearn} & 99 & 0.876 & 0.139 &  & \textbf{AutoSKLearn} & 99 & 0.887 & 0.130 \\ \cline{2-5} \cline{7-10} 
 & \textbf{SmartML} & 90 & 0.808 & 0.199 &  & \textbf{SmartML} & 89 & 0.826 & 0.169 \\ \cline{2-5} \cline{7-10} 
 & \textbf{SmartML-e} & 96 & 0.838 & 0.159 &  & \textbf{SmartML-e} & 95 & 0.840 & 0.165 \\ \cline{2-5} \cline{7-10} 
\multirow{-9}{*}{\textbf{30 Min}} & \textbf{TPOT} & 59 & 0.885 & 0.136 & \multirow{-9}{*}{\textbf{240 Min}} & \textbf{TPOT} & 89 & 0.893 & 0.126 \\ \hline
\end{tabular}}
\label{tab:GeneralSummary}
\end{table}

% \begin{table}[!ht]
% \centering
% \caption{Average performance of the frameworks per time budget}
% % \resizebox{0.9\textwidth}{!}
% {\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{EFEFEF}\cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} } &  &  & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Gain (Accuracy)}} & \multicolumn{3}{c}{\textbf{\#datasets with gain}} & \multicolumn{2}{c}{\textbf{Loss (Accuracy)}} \\
% \multirow{-2}{*}{\rowcolor[HTML]{EFEFEF}\cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} \textbf{Time Budget}}} & \multirow{-2}{*}{\textbf{Framework}} & \multirow{-2}{*}{\textbf{N}} & \textbf{Mean} & \textbf{SD} &  \textbf{Mean} & \textbf{Max} & \textbf{ > 1\%} & \textbf{ $\approx 0 \%$} & \textbf{ < 1\%} & \textbf{Mean} & \textbf{Max} \\ \hline
%  & \textbf{ATM} & 75 & 0.888 & 0.123   & & & &  & & & \\ \cline{2-12}  
%  & \textbf{AutoWeka} & 86 & 0.848 & 0.161  & & & &  & & & \\ \cline{2-12} 
%  & \textbf{Recipe} & 33 & 0.840 & 0.176   & & & &  & & & \\ \cline{2-12} 
%  & \textbf{AutoSKLearn-e} & 99 & 0.873 & 0.139  & & & &  & & & \\ \cline{2-12} 
%  & \textbf{AutoSKLearn-m} & 99 & 0.870 & 0.144  & & & &  & & & \\ \cline{2-12}
%  & \textbf{AutoSKLearn-v} & 99 & 0.868 & 0.145  & & & &  & & & \\ \cline{2-12} 
%  & \textbf{AutoSKLearn} & 99 & 0.873 & 0.143 & & & &  & & & \\ \cline{2-12} 
%  & \textbf{SmartML} & 89 & 0.799 & 0.212  & & & &  & & & \\ \cline{2-12}
% \multirow{-9}{*}{\textbf{10 Min}} & \textbf{TPOT} & 43 & 0.894 & 0.117  & & & & & & & \\ \hline
%  & \textbf{ATM} & 74 & 0.903 & 0.116 & & & &  & & & \\ \cline{2-12} 
%  & \textbf{AutoWeka} & 90 & 0.845 & 0.161 & & & &  & & & \\ \cline{2-12} 
%  & \textbf{Recipe} & 69 & 0.855 & 0.144 & & & &  & & & \\ \cline{2-12} 
%  & \textbf{AutoSKLearn-e} & 99 & 0.880 & 0.136  & & & &  & & & \\ \cline{2-12}
%  & \textbf{AutoSKLearn-m} & 99 & 0.873 & 0.143  & & & &  & & & \\ \cline{2-12} 
%  & \textbf{AutoSKLearn-v} & 99 & 0.873 & 0.142  & & & &  & & & \\ \cline{2-12} 
%  & \textbf{AutoSKLearn} & 99 & 0.876 & 0.139 & & & &  & & & \\ \cline{2-12}  
%  & \textbf{SmartML} & 90 & 0.808 & 0.199 & & & &  & & & \\ \cline{2-12} 
% \multirow{-9}{*}{\textbf{30 Min}} & \textbf{TPOT} & 59 & 0.885 & 0.136  & & & & & & & \\ \hline

% & \textbf{ATM} & 79 & 0.890 & 0.126 & & & &  & & & \\ \cline{2-12} 
% & \textbf{AutoWeka} & 91 & 0.844 & 0.157 & & & &  & & & \\ \cline{2-12} 
% & \textbf{Recipe} & 76 & 0.864 & 0.139 & & & &  & & & \\ \cline{2-12} 
% & \textbf{AutoSKLearn-e} & 99 & 0.884 & 0.132 & & & &  & & & \\ \cline{2-12} 
% & \textbf{AutoSKLearn-m} & 99 & 0.873 & 0.141 & & & &  & & & \\ \cline{2-12}  
% & \textbf{AutoSKLearn-v} & 99 & 0.874 & 0.137 & & & &  & & & \\ \cline{2-12}  
% & \textbf{AutoSKLearn} & 99 & 0.882 & 0.133 & & & &  & & & \\ \cline{2-12} 
% & \textbf{SmartML} & 89 & 0.816 & 0.194 & & & &  & & & \\ \cline{2-12} 
% \multirow{-9}{*}{\textbf{60 Min}} & \textbf{TPOT} & 70 & 0.890 & 0.131  & & & & & & & \\ \hline
% & \textbf{ATM} & 86 & 0.895 & 0.123 & & & &  & & & \\ \cline{2-12}
% & \textbf{AutoWeka} & 96 & 0.845 & 0.159 & & & &  & & & \\ \cline{2-12} 
% & \textbf{Recipe} & 85 & 0.859 & 0.155 & & & &  & & & \\ \cline{2-12}  
% & \textbf{AutoSKLearn-e} & 99 & 0.886 & 0.130 & & & &  & & & \\ \cline{2-12} 
% & \textbf{AutoSKLearn-m} & 99 & 0.877 & 0.136 & & & &  & & & \\ \cline{2-12} 
% & \textbf{AutoSKLearn-v} & 99 & 0.875 & 0.141 & & & &  & & & \\ \cline{2-12}
% & \textbf{AutoSKLearn} & 99 & 0.887 & 0.130 & & & &  & & & \\ \cline{2-12} 
% & \textbf{SmartML} & 89 & 0.826 & 0.169 & & & &  & & & \\ \cline{2-12}
% \multirow{-9}{*}{\textbf{240 Min}} & \textbf{TPOT} & 89 & 0.893 & 0.126  & & & & & & & \\ \hline
% \end{tabular}}
% \label{tab:GeneralSummary}
% \end{table}

==> tables/wilcoxon-10min.tex <==
\begin{table*}[!ht]
\centering\scriptsize
\caption{Wilcoxon pairwise test p-values for AutoML frameworks over different time budgets. Bold entries highlight significant differences ($p\leq 0.05$) and highlighted entries in each row represents a given AutoML framework (row) outperforms another AutoML framework (column).}  

\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
\hline
\multicolumn{10}{c}{\textbf{\LARGE 10 Minutes}}\\
\hline
& ATM & AutoWeka & Recipe & AutoSKLearn-e &   AutoSKLearn-m & AutoSKLearn-v &  AutoSKLearn & SmartML & SmartML-e &  TPOT \\

\hline
ATM &  \cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.046}&0.313&0.965&0.557&0.527&0.446&\cellcolor{blue!25}\textbf{0.044}&\cellcolor{blue!25}\textbf{0.035}&0.597\\
\hline
AutoWeka &  \textbf{0.046}&\cellcolor{black!25}{}&0.797&\textbf{0.0}&\textbf{0.0}&\textbf{0.002}&\textbf{0.0}&0.796&0.389&0.085\\
\hline
Recipe &  0.313&0.797&\cellcolor{black!25}{}&0.024&0.072&0.399&\textbf{0.004}&0.214&0.911&0.386\\
\hline
AutoSKLearn-e &  0.965&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.024}&\cellcolor{black!25}{}&0.941&\cellcolor{blue!25}\textbf{0.015}&\cellcolor{blue!25}\textbf{0.006}&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{blue!25}\textbf{0.008}&0.758\\
\hline
AutoSKLearn-m &  0.557&\cellcolor{blue!25}\textbf{0.0}&0.072&0.941&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.011}&\textbf{0.008}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.002}&0.288\\
\hline
AutoSKLearn-v & 0.527&\cellcolor{blue!25}\textbf{0.002}&0.399&0.015&\textbf{0.011}&\cellcolor{black!25}{}&\textbf{0.0}&\cellcolor{blue!25}\textbf{0.004}&0.118&\cellcolor{blue!25}\textbf{0.024}\\
\hline
AutoSKLearn & 0.446&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.004}&\textbf{0.006}&\cellcolor{blue!25}\textbf{0.008}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.001}&0.491\\
\hline
SmartML &  \textbf{0.044}&0.796&0.214&\textbf{0.001}&\textbf{0.0}&\textbf{0.004}&\textbf{0.0}&\cellcolor{black!25}{}&\textbf{0.014}&\textbf{0.002}\\
\hline
SmartML-e & \textbf{0.035}&0.389&0.911&\textbf{0.008}&\textbf{0.002}&0.118&\textbf{0.001}&\cellcolor{blue!25}\textbf{0.014}&\cellcolor{black!25}{}&0.076\\
\hline

TPOT & 0.597&0.085&0.386&0.758&0.288&0.024&0.491&\cellcolor{blue!25}\textbf{0.002}&0.076&\cellcolor{black!25}{}\\
\hline
\multicolumn{10}{c}{\textbf{\LARGE 30 Minutes}}\\
\hline
& ATM & AutoWeka & Recipe & AutoSKLearn-e &   AutoSKLearn-m & AutoSKLearn-v &  AutoSKLearn & SmartML & SmartML-e &  TPOT \\

\hline
ATM & 
\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.021}&0.26&0.981&0.283&0.136&0.883&\cellcolor{blue!25}\textbf{0.002}&\cellcolor{blue!25}\textbf{0.002}&0.87\\
\hline
AutoWeka & 
\textbf{0.021}&\cellcolor{black!25}{}&0.697&\textbf{0.0}&\textbf{0.0}&\textbf{0.003}&\textbf{0.0}&0.356&0.656&\textbf{0.001}\\
\hline
Recipe & 
0.26&0.697&\cellcolor{black!25}{}&\textbf{0.0}&\textbf{0.002}&\textbf{0.048}&\textbf{0.0}&\cellcolor{blue!25}\textbf{0.021}&0.639&\textbf{0.0}\\
\hline
AutoSKLearn-e & 
0.981&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{blue!25}\textbf{0.0}&0.209&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.921\\
\hline
AutoSKLearn-m & 
0.283&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.002}&\textbf{0.00}1&\cellcolor{black!25}{}&0.093&0.137&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.004}&0.124\\
\hline
AutoSKLearn-v & 
0.136&\cellcolor{blue!25}\textbf{0.003}&\cellcolor{blue!25}\textbf{0.048}&\textbf{0.0}&0.093&\cellcolor{black!25}{}&\textbf{0.002}&\cellcolor{blue!25}\textbf{0.007}&\cellcolor{blue!25}\textbf{0.024}&\textbf{0.002}\\
\hline
AutoSKLearn & 
0.883&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.209&0.137&\cellcolor{blue!25}\textbf{0.002}&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.001}&0.137\\
\hline
SmartML & 
\textbf{0.002}&0.356&\textbf{0.021}&\textbf{0.0}&\textbf{0.0}&\textbf{0.007}&\textbf{0.0}&\cellcolor{black!25}{}&\textbf{0.015}&\textbf{0.0}\\
\hline
SmartML-e & 
\textbf{0.002}&0.656&0.639&\textbf{0.0}&\textbf{0.004}&\textbf{0.024}&\textbf{0.001}&\cellcolor{blue!25}\textbf{0.015}&\cellcolor{black!25}{}&\textbf{0.001}\\
\hline
TPOT & 
0.87&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{blue!25}\textbf{0.0}&0.921&0.124&\cellcolor{blue!25}\textbf{0.002}&0.137&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{black!25}{}\\
\hline
\multicolumn{10}{c}{\textbf{\LARGE 60 Minutes}}\\
\hline
& ATM & AutoWeka & Recipe & AutoSKLearn-e &   AutoSKLearn-m & AutoSKLearn-v &  AutoSKLearn & SmartML & SmartML-e &  TPOT \\

\hline
ATM & 
\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.006}&0.176&0.083&0.482&0.585&0.14&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{blue!25}\textbf{0.001}&0.093\\
\hline
AutoWeka & 
\textbf{0.006}&\cellcolor{black!25}{}&0.397&\textbf{0.0}&\textbf{0.0}&\textbf{0.0}&\textbf{0.0}&0.759&0.328&\textbf{0.0}\\
\hline
Recipe & 
0.176&0.397&\cellcolor{black!25}{}&\textbf{0.0}&\textbf{0.025}&\textbf{0.01}&\textbf{0.0}&\cellcolor{blue!25}\textbf{0.014}&0.609&\textbf{0.0}\\
\hline
AutoSKLearn-e & 
0.083&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.007}&\cellcolor{blue!25}\textbf{0.001}&0.326&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.001}&0.352\\
\hline
AutoSKLearn-m & 
0.482&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.025}&0.007&\cellcolor{black!25}{}&0.545&0.0&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{blue!25}\textbf{0.006}&0.027\\
\hline
AutoSKLearn-v & 
0.585&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.01}&\textbf{0.001}&0.545&\cellcolor{black!25}{}&\textbf{0.0}&\cellcolor{blue!25}\textbf{0.002}&\cellcolor{blue!25}\textbf{0.026}&\textbf{0.007}\\
\hline
AutoSKLearn & 
0.14&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.326&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.689\\
\hline
SmartML & 
\textbf{0.001}&0.759&\textbf{0.014}&\textbf{0.0}&\textbf{0.001}&\textbf{0.002}&\textbf{0.0}&\cellcolor{black!25}{}&\textbf{0.047}&\textbf{0.0}\\
\hline
SmartML-e & 
\textbf{0.001}&0.328&0.609&\textbf{0.001}&\textbf{0.006}&\textbf{0.026}&\textbf{0.0}&\cellcolor{blue!25}\textbf{0.047}&\cellcolor{black!25}{}&\textbf{0.001}\\
\hline
TPOT & 
0.093&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.352&\cellcolor{blue!25}\textbf{0.027}&\cellcolor{blue!25}\textbf{0.007}&0.689&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{black!25}{}\\
\hline
\multicolumn{10}{c}{\textbf{\LARGE 4 Hours}}\\
\hline
& ATM & AutoWeka & Recipe & AutoSKLearn-e &   AutoSKLearn-m & AutoSKLearn-v &  AutoSKLearn & SmartML & SmartML-e &  TPOT \\

\hline
ATM & 
\cellcolor{black!25}{}&0.065&0.101&0.535&0.877&0.788&0.561&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{blue!25}\textbf{0.017}&0.092\\
\hline
AutoWeka & 
0.065&\cellcolor{black!25}{}&0.893&\textbf{0.0}&\textbf{0.0}&\textbf{0.002}&\textbf{0.0}&0.243&0.892&\textbf{0.0}\\
\hline
Recipe & 
0.101&0.893&\cellcolor{black!25}{}&\textbf{0.0}&\textbf{0.002}&\textbf{0.0}&\textbf{0.0}&0.052&0.383&\textbf{0.0}\\
\hline
AutoSKLearn-e & 
0.535&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.006}&\cellcolor{blue!25}\textbf{0.016}&0.477&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.001}&0.139\\
\hline
AutoSKLearn-m & 
0.877&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.002}&\textbf{0.006}&\cellcolor{black!25}{}&0.957&\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.002}&\textbf{0.001}\\
\hline
AutoSKLearn-v & 
0.788&\cellcolor{blue!25}\textbf{0.002}&\cellcolor{blue!25}\textbf{0.0}&\textbf{0.016}&0.957&\cellcolor{black!25}{}&0.0&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.003}&\textbf{0.0}\\
\hline
AutoSKLearn & 
0.561&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.477&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{black!25}{}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.156\\
\hline
SmartML & 
\textbf{0.001}&0.243&0.052&\textbf{0.0}&\textbf{0.0}&\textbf{0.0}&\textbf{0.0}&\cellcolor{black!25}{}&\textbf{0.031}&\textbf{0.0}\\
\hline
SmartML-e & 
\textbf{0.017}&0.892&0.383&\textbf{0.001}&\textbf{0.002}&\textbf{0.003}&\textbf{0.0}&\cellcolor{blue!25}\textbf{0.031}&\cellcolor{black!25}{}&\textbf{0.0}\\
\hline
TPOT & 
0.092&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&0.139&\cellcolor{blue!25}\textbf{0.001}&\cellcolor{blue!25}\textbf{0.0}&0.156&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{blue!25}\textbf{0.0}&\cellcolor{black!25}{}\\
\hline
\bottomrule

\end{tabular}}
\label{table:10-min_wilcoxon_matrix}
\end{table*}

==> tables/wilcoxon-time.tex <==
\begin{table}[!t]
\centering
\caption{Wilcoxon test p-values for all the AutoML frameworks over different time budgets. Bold entries highlight significant difference.}
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|ccccc}
\hline
\rowcolor[HTML]{656565} 
\cellcolor[HTML]{343434}{\color[HTML]{FFFFFF} \textbf{Framework}} & {\color[HTML]{FFFFFF} \textbf{Time Budget 1}} & {\color[HTML]{FFFFFF} \textbf{Time Budget 2}} & {\color[HTML]{FFFFFF} \textbf{Avg. Acc. Diff}} & {\color[HTML]{FFFFFF} \textbf{$P$ value}} & \multicolumn{1}{c|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{Framework}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{656565}{\color[HTML]{FFFFFF} \textbf{Time Budget 1}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{656565}{\color[HTML]{FFFFFF} \textbf{Time Budget 2}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{656565}{\color[HTML]{FFFFFF} \textbf{Avg. Acc. Diff}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{656565}{\color[HTML]{FFFFFF} \textbf{$P$ value}}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{AutoWeka} & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.031 & \cellcolor[HTML]{EFEFEF}\textbf{0.005} & \multicolumn{1}{c|}{\textbf{AutoSKLearn}} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.003} & \multicolumn{1}{c|}{0.362} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{AutoWeka} & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.038 & \cellcolor[HTML]{EFEFEF}\textbf{0.037} & \multicolumn{1}{c|}{\textbf{AutoSKLearn}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.009} & \multicolumn{1}{c|}{\textbf{0.000}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{AutoWeka} & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}0.008 & \cellcolor[HTML]{EFEFEF}0.658 & \multicolumn{1}{c|}{\textbf{AutoSKLearn}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{0.005} & \multicolumn{1}{c|}{\textbf{0.019}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{AutoWeka} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.083 & \cellcolor[HTML]{EFEFEF}\textbf{0.000} & \multicolumn{1}{c|}{\textbf{AutoSKLearn}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.014} & \multicolumn{1}{c|}{\textbf{0.001}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{AutoWeka} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}0.051 & \cellcolor[HTML]{EFEFEF}\textbf{0.022} & \multicolumn{1}{c|}{\textbf{AutoSKLearn}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{0.011} & \multicolumn{1}{c|}{\textbf{0.002}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{AutoWeka} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}0.044 & \cellcolor[HTML]{EFEFEF}\textbf{0.004} & \multicolumn{1}{c|}{\textbf{AutoSKLearn}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{0.005} & \multicolumn{1}{c|}{0.117} \\ \hline
\textbf{TPOT} & 30 & 10 & 0.009 & 0.165 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-v}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}30} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.005} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.226} \\ \hline
\textbf{TPOT} & 60 & 10 & 0.008 & 0.399 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-v}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}60} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.007} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.004}} \\ \hline
\textbf{TPOT} & 60 & 30 & 0.001 & 0.400 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-v}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}60} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}30} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.002} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.141} \\ \hline
\textbf{TPOT} & 240 & 10 & 0.013 & \textbf{0.013} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-v}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}240} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.007} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.000}} \\ \hline
\textbf{TPOT} & 240 & 30 & 0.006 & \textbf{0.027} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-v}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}240} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}30} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.002} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0.027}} \\ \hline
\textbf{TPOT} & 240 & 60 & 0.004 & \textbf{0.010} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-v}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}240} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}60} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.000} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.110} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Recipe} & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}-0.031 & \cellcolor[HTML]{EFEFEF}0.272 & \multicolumn{1}{c|}{\textbf{AutoSKLearn-e}} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.007} & \multicolumn{1}{c|}{\textbf{0.000}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Recipe} & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.014 & \cellcolor[HTML]{EFEFEF}0.067 & \multicolumn{1}{c|}{\textbf{AutoSKLearn-e}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.011} & \multicolumn{1}{c|}{\textbf{0.000}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Recipe} & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}0.007 & \cellcolor[HTML]{EFEFEF}0.829 & \multicolumn{1}{c|}{\textbf{AutoSKLearn-e}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{0.004} & \multicolumn{1}{c|}{0.675} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Recipe} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.026 & \cellcolor[HTML]{EFEFEF}\textbf{0.010} & \multicolumn{1}{c|}{\textbf{AutoSKLearn-e}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.013} & \multicolumn{1}{c|}{\textbf{0.000}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Recipe} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}0.005 & \cellcolor[HTML]{EFEFEF}0.650 & \multicolumn{1}{c|}{\textbf{AutoSKLearn-e}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{0.006} & \multicolumn{1}{c|}{\textbf{0.038}} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Recipe} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}-0.001 & \cellcolor[HTML]{EFEFEF}0.939 & \multicolumn{1}{c|}{\textbf{AutoSKLearn-e}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{0.002} & \multicolumn{1}{c|}{0.265} \\ \hline
\textbf{ATM} & 30 & 10 & 0.007 & 0.341 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-m}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}30} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.004} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.211} \\ \hline
\textbf{ATM} & 60 & 10 & 0.009 & 0.488 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-m}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}60} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.004} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.198} \\ \hline
\textbf{ATM} & 60 & 30 & 0.009 & 0.538 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-m}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}60} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}30} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.00} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.956} \\ \hline
\textbf{ATM} & 240 & 10 & 0.026 & 0.594 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-m}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}240} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}10} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.008} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.099} \\ \hline
\textbf{ATM} & 240 & 30 & 0.025 & 0.964 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-m}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}240} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}30} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.004} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.614} \\ \hline
\textbf{ATM} & 240 & 60 & 0.015 & 0.496 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{AutoSKLearn-m}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}240} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}60} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.004} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.398} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{SmartML} & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.007 & \cellcolor[HTML]{EFEFEF}0.636 & \multicolumn{1}{c|}{\textbf{SmartML-e}} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.008} & \multicolumn{1}{c|}{0.521} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{SmartML} & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.009 & \cellcolor[HTML]{EFEFEF}0.832 & \multicolumn{1}{c|}{\textbf{SmartML-e}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.003} & \multicolumn{1}{c|}{0.589} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{SmartML} & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}0.009 & \cellcolor[HTML]{EFEFEF}0.597 & \multicolumn{1}{c|}{\textbf{SmartML-e}} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{-0.004} & \multicolumn{1}{c|}{0.672} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{SmartML} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}10 & \cellcolor[HTML]{EFEFEF}0.026 & \cellcolor[HTML]{EFEFEF}0.121 & \multicolumn{1}{c|}{\textbf{SmartML-e}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{0.011} & \multicolumn{1}{c|}{0.092} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{SmartML} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}30 & \cellcolor[HTML]{EFEFEF}0.025 & \cellcolor[HTML]{EFEFEF}\textbf{0.050} & \multicolumn{1}{c|}{\textbf{SmartML-e}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{0.004} & \multicolumn{1}{c|}{0.182} \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{SmartML} & \cellcolor[HTML]{EFEFEF}240 & \cellcolor[HTML]{EFEFEF}60 & \cellcolor[HTML]{EFEFEF}0.015 & \cellcolor[HTML]{EFEFEF}0.071 & \multicolumn{1}{c|}{\textbf{SmartML-e}} & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{60} & \multicolumn{1}{c|}{0.008} & \multicolumn{1}{c|}{0.305} \\ \hline
\end{tabular}}

\label{tab:wilcoxon_timebudget}
\end{table}
